Fisher Information of Scale

Motivated by the information bound for the asymptotic variance of M-estimates for scale, we define Fisher information of scale of any distribution function F on the real line as a suitable supremum. In addition, we enforce equivariance by a scale factor. Fisher information of scale is weakly lower semicontinuous and convex. It is finite iff the usual assumptions on densities hold, under which Fisher information of scale is classically defined, and then both classical and our notions agree. Fisher information of scale finite is also equivalent to L_2-differentiability and local asymptotic normality, respectively, of the scale model induced by F.

==> Fiskdef2.tex <==
%\documentclass[authoryear,preprint,review,12pt]{elsarticle}
%\documentclass[authoryear,hyperref,final,3p]{elsarticle}
%\documentclass[authoryear,hyperref,preprint,1p]{elsarticle}
%
%\smartqed  % flush right qed marks, e.g. at end of proof
%
\usepackage{graphicx}

%--------------------------------------------------------------------------------------
% Packages used by authors:
%--------------------------------------------------------------------------------------
\usepackage{amsmath}
\usepackage{subfigure}
\usepackage{amssymb}
\usepackage{mathptmx}      % use Times fonts if available on your TeX system

\RequirePackage{natbib}
\RequirePackage{hypernat}
\usepackage{url}
%\RequirePackage[hyperindex,backref,bookmarks,bookmarksnumbered,plainpages=false]{hyperref}
\RequirePackage[hyperindex,bookmarks,bookmarksnumbered,plainpages=false]{hyperref}
%alternatively:
%\newcommand{\href}[2]{{#2}}
\RequirePackage{ifthen}

%--------------------------------------------------------------------------------------
% New commands
% -----------------------------------------------------------------------
\newcommand{\Ds}{\displaystyle} \newcommand{\Ts}{\textstyle}
\newcommand{\Ss}{\scriptstyle}  \newcommand{\SSs}{\scriptscriptstyle}
\newcommand{\ssr}{\rm\scriptscriptstyle}
%--------------------------------------------------------------------------------------
\newcommand{\req}{\relax}
\newcommand{\rfia}[1]{\makebox[\parindent][l]{%
                     \makebox[0em][r]{\rm(}\sf#1\rm)}}
\newcounter{ABCcB}\renewcommand{\theABCcB}{\theThm~(\alph{ABCcB})}
\newcommand{\theABCcC}{\alph{ABCcB}}

\newenvironment{ABCTH}{\begin{list}{%    VE LABELWIDTH 1em + LABELSEP 0.5em
  \rfia{\theABCcC}}{\usecounter{ABCcB} \topsep 0ex \partopsep 0ex \itemsep0ex
  \parsep=\parskip \leftmargin 0em \rightmargin 0em \itemindent=\parindent
  \listparindent=\parindent  \labelsep 0.5em \labelwidth 0.5em }}{\end{list}}

\newcommand{\Ew}{\mathop{\rm {{}E{}}}\nolimits} % mathop erkennt nur (
\newcommand{\Var}{\mathop{\rm Var}\nolimits}    % extra \,space
\newcommand{\ve}{\varepsilon}
\newcommand{\IF}{\mathop{\rm IF}\nolimits}
\newcommand{\Lw}{{\cal L}}
\newcommand{\Lo}{\mathop{\rm {{}o{}}}\nolimits}
\newcommand{\LO}{\mathop{\rm {{}O{}}}\nolimits}
\newcommand{\asVar}{\mathop{\rm{} asVar{}}\nolimits}
\newcommand{\asMSE}{\mathop{\rm{} asMSE{}}\nolimits}
\newcommand{\asBias}{\mathop{\rm{} asBias{}}\nolimits}
\newcommand{\argmin}{\mathop{\rm{} argmin{}}}
\newcommand{\tr}{\mathop{\rm{} tr{}}}
\newcommand{\B}{\mathbb B}
\newcommand{\C}{\mathbb C}
\newcommand{\R}{\mathbb R}
\newcommand{\Rq}{\bar{\mathbb R}}
\newcommand{\Bq}{\bar{\mathbb B}}
\newcommand{\Q}{\mathbb Q}
\newcommand{\Z}{\mathbb Z}
\newcommand{\N}{\mathbb N}
\newcommand{\Jc}{\mathop{\bf\rm{{}I{}}}\nolimits}
\newcommand{\EM} {{\mathbb I}}
\newcommand{\sB}{{\Ss \mathbb B}}
\newcommand{\sC}{{\Ss \mathbb C}}
\newcommand{\sR}{{\Ss \mathbb R}}
\newcommand{\sRq}{\bar{\Ss \mathbb R}}
\newcommand{\sQ}{{\Ss \mathbb Q}}
\newcommand{\sZ}{{\Ss \mathbb Z}}
\newcommand{\sN}{{\Ss \mathbb N}}
\newcommand{\sEM} {{\Ss \mathbb I}}
\newcommand{\hEM}{{\mbox{\hMtenmsbm I}}}  % Emat \magstephalf(11pt)
\newcommand{\oEM}{{\mbox{\oMtenmsbm I}}}  % Emat \magstepone(12pt)
\newcommand{\iid}{\mathrel{\stackrel{\ssr i.i.d.}{\sim}}}
\newcommand{\also}{\Longrightarrow}
\newcommand{\Tfrac}[2]{\textstyle\frac{#1}{#2}}
\newcommand{\Tint}{\mathop{\Ts\int}\nolimits}
% -----------------------------------------------------------------------
\newlength{\weit} \newlength{\lang} \newlength{\hoch} \newlength{\breit}
\newlength{\SyW} \newlength{\SyyW}  \newlength{\msu}  \msu=\mathsurround % \AzP=\msu gesetzt
\newcommand{\weg}{\hspace{\msu}}\newcommand{\ran}{\hspace{-\mathsurround}}
\newcommand{\wto}{\mathrel{\mathsurround0em \mbox{$\longrightarrow$}%
  \llap{\settowidth{\SyW}{$\longrightarrow$}%             \protect in @{}
  \raisebox{-.15ex}{\makebox[\SyW]{\scriptsize\rm w}}}}}
\newcommand{\gwto}{\mathrel{\mathsurround0em \mbox{$\ggrto$}%
  \llap{\settowidth{\SyW}{$\ggrto$}%                      \protect in @{}
  \raisebox{-.15ex}{\makebox[\SyW]{\scriptsize\rm w}}}}}
\newcommand{\vto}{\mathrel{\mathsurround0em \mbox{$\longrightarrow$}%
  \llap{\settowidth{\SyW}{$\longrightarrow$}%             \protect in @{}
  \raisebox{-.15ex}{\makebox[\SyW]{\scriptsize\rm v}}}}}
% -----------------------------------------------------------------------
\newtheorem{Thm}{Theorem}%[section]   % STARTS each SECTION
\newtheorem{Prop}[Thm]{Proposition}
\newtheorem{Lem}[Thm]{Lemma}
\newtheorem{Rem}[Thm]{Remark}
\newtheorem{Cor}[Thm]{Corollary}
\newtheorem{Def}[Thm]{Definition}
\newtheorem{Algo}[Thm]{Algorithm}
\newcommand{\nquad}{\!\!\!\!}
\newcommand{\mparagraph}[1]{\vspace{0.1ex}\noindent\textbf{#1}}
\numberwithin{equation}{section}
\numberwithin{Thm}{section}
\newcommand{\uP}{\vspace{-3ex}}
\newcommand{\Bullet}{{\centerdot}}
\newcounter{ABCc}
\renewcommand{\theABCc}{\alph{ABCc}}
\newenvironment{ABC}{\begin{list}{%    VE LABELWIDTH 1em + LABELSEP 0.5em
  \rfia{\theABCc}}{\usecounter{ABCc} \topsep 0ex \partopsep 0ex \itemsep0ex
  \parsep=\parskip \leftmargin 0em \rightmargin 0em \itemindent=\parindent
  \listparindent=\parindent  \labelsep 0.5em \labelwidth 0.5em }}{\end{list}}
\newcommand{\seitref}{}
\newcommand{\unpub}{Unpublished discussion paper}
\newcommand{\unpubsem}{Unpublished manuscript}
\newcommand{\accepted}{accepted by }
\newcommand{\Contribution}{Contribution to }
%\newcommand{\accepted}{accepted by}
\newcommand{\unpM}{unpublished discussion paper}

% Insert the name of "your journal" with
% \journalname{AStA Advances in Statistical Analysis}
\journal{Statistics and Probability Letters}
%

